Natural Language Interfaces for Tabular Data Querying and Visualization: A Survey

The emergence of natural language processing has revolutionized the way users interact with tabular data, enabling a shift from traditional query languages and manual plotting to more intuitive, language-based interfaces. The rise of large language models (LLMs) such as ChatGPT and its successors has further advanced this field, opening new avenues for natural language processing techniques. This survey presents a comprehensive overview of natural language interfaces for tabular data querying and visualization, which allow users to interact with data using natural language queries. We introduce the fundamental concepts and techniques underlying these interfaces with a particular emphasis on semantic parsing, the key technology facilitating the translation from natural language to SQL queries or data visualization commands. We then delve into the recent advancements in Text-to-SQL and Text-to-Vis problems from the perspectives of datasets, methodologies, metrics, and system designs. This includes a deep dive into the influence of LLMs, highlighting their strengths, limitations, and potential for future improvements. Through this survey, we aim to provide a roadmap for researchers and practitioners interested in developing and applying natural language interfaces for data interaction in the era of large language models.

==> tikz/ontology.tex <==
\begin{tikzpicture}[grow'=right,level distance=6.0in,sibling distance=.22in]
\tikzset{
  treenode/.style = {shape=rectangle, rounded corners,
                     draw, align=center,
                     top color=white, bottom color=blue!20, inner sep=12pt,level distance = 20em},
  edge from parent/.style= 
            {thick, draw, edge from parent fork right},
  root/.style     = {treenode, font=\Huge, bottom color=orange!10},
  l1/.style      = {treenode, font=\Huge, minimum width=1.4in, bottom color=orange!20},
  l2/.style      = {treenode, font=\Huge, minimum width=1.4in, bottom color=orange!30},
  l3/.style      = {treenode, font=\Huge, minimum width=1.6in, bottom color=orange!40, level distance = 15em},
  l4/.style      = {treenode, font=\Huge, minimum width=1.3in, bottom color=orange!50},
  l2w/.style      = {treenode, font=\Huge, minimum width=1.2in,text width=1.1in, bottom color=white},
  ppl/.style      = {treenode, font=\Huge, bottom color=orange!100},
  pplw/.style      = {treenode, font=\Huge, minimum width=1.5in, bottom color=white},
  wd15/.style      = {treenode, font=\Huge, minimum width=1.5in, bottom color=white},
  wd14/.style      = {treenode, font=\Huge, minimum width=1.4in, bottom color=white},
  wd13/.style      = {treenode, font=\Huge, minimum width=1.3in, bottom color=white},
  wd12/.style      = {treenode, font=\Huge, minimum width=1.2in, bottom color=white},
  wd7/.style      = {treenode, font=\Huge, minimum width=0.7in, bottom color=white},
  dummy/.style    = {circle,draw},
  adj/.style      = {treenode, font=\Huge, minimum width=1.3in, bottom color=orange!50, xshift=-5cm},
  adjnew/.style      = {treenode, font=\Huge, minimum width=1.3in, bottom color=orange!50, xshift=-10cm},
  adj1/.style      = {treenode, font=\Huge, minimum width=1.3in, bottom color=orange!50},
  %       every tree node/.style=             {draw,minimum width=1in,text width=1in,align=center}
  }
  
\Tree 
    [. \node[root] {VLPMs}; 
        [. \node [l1,anchor=west,xshift=-6cm] {Input Data Encoding};
              [. \node[l2,anchor=west,xshift=-8cm] {Language Encoding};
                [. \node[l2,anchor=west,xshift=-10cm] {Language Representation};
                   [. \node[ppl,anchor=west,xshift=-10cm] {Bert-formatted Input Representation};
                   ]
                ]
                [. \node[l2,anchor=west,xshift=-10cm] {Intra-modality Processing (if used)};
                   [. \node[ppl,anchor=west,xshift=-10cm] {Transformer Encoder(s)};
                   ]
                ]
              ]
              [. \node [l1,anchor=west,xshift=-8cm] {Vision Encoding};
              [. \node[l2,anchor=west,xshift=-11cm] {Visual  Representation};
                    [. \node[l3,anchor=west,xshift=-15cm] {Bert-style sequential representation};
                      [. \node[l4,anchor=west,xshift=-15cm] {Granularity};
                        [. \node[ppl,anchor=west,xshift=-19cm] {RoIs};
                        ]
                        [. \node[ppl,anchor=west,xshift=-19cm] {Patches};
                        ]
                        [. \node[ppl,anchor=west,xshift=-19cm] {Pixels};
                        ]
                        [. \node[ppl,anchor=west,xshift=-19cm] {Images};
                        ]
                      ]
                     ]
              ]
              [. \node[l2,anchor=west,xshift=-11cm] {Intra-modality Processing (If Used)};
                 [. \node[ppl,anchor=west,xshift=-11cm] {Transformer Encoder(s)};
                 ]
                 [. \node[ppl,anchor=west,xshift=-11cm] {Non-Transformer};
                 ]
              ]
             ]
        ]
        [. \node [l1,anchor=west,xshift=-6cm] {Model Structure};
            [. \node [l1,anchor=west,xshift=-9cm] {V-L Interaction Model (V-LIM)};
                [. \node[ppl,anchor=west,xshift=-9cm] {Self-attention-based V-LIM};
                ]
                [. \node[ppl,anchor=west,xshift=-9cm] {Co-attention-based V-LIM};
                ]
                [. \node[ppl,anchor=west,xshift=-9cm] {VSE-based V-LIM (Dual Encoder Method)}; 
                ]
            ]
            [. \node [l1,anchor=west,xshift=-9cm] {Modality Processing Type};
                [. \node[ppl,anchor=west,xshift=-10cm] {Single-stream};
                ]
                [. \node[ppl,anchor=west,xshift=-10cm] {Double-stream}; 
                ]
            ]
        ]
        [. \node [l1,anchor=west,xshift=-6cm] {Pre-training};
            [. \node[l2,anchor=west,xshift=-9cm] {Datasets(DTs)}; 
              [. \node[ppl,anchor=west,xshift=-10cm] {Webly Collected};
              ]
              [. \node[ppl,anchor=west,xshift=-10cm] {In-Domain + Out-of-Domain};
              ]
              [. \node[ppl,anchor=west,xshift=-10cm] {Tasks/domain-specific DT(s) Only};
              ]
              [. \node[ppl,anchor=west,xshift=-10cm] {Auxiliary Single-modality DT(s)};
              ]
            ]
            [. \node[l3,anchor=west,xshift=-9cm] {Tasks and Objectives}; 
              [. \node[l3,anchor=west,xshift=-9cm] {Cross-modal Tasks, Objectives};
                [. \node[ppl,anchor=west,xshift=-10cm] {Cross-modal Masked Language Modeling (CMLM), NLL};
                ]
                [. \node[l4,anchor=west,xshift=-10cm] {Cross-modal Masked Region Modeling (CMRM)};
                   [. \node[ppl,anchor=west,xshift=-6cm] {CMRM\textsubscript{C}, CE};
                   ]
                   [. \node[ppl,anchor=west,xshift=-6cm] {CMRM\textsubscript{D}, KL Divergence};
                   ]
                   [. \node[ppl,anchor=west,xshift=-6cm] {CMRM\textsubscript{R}, L2};
                   ]
                ]
                [. \node[l4,anchor=west,xshift=-10cm] {Cross-modal Alignment (CA)};
                      [. \node[ppl,anchor=west,xshift=-9cm] {Matching-based CA, BCE};
                      ]
                      [. \node[ppl,anchor=west,xshift=-9cm] {Ranking-based CA, Contrastive};
                      ]
                ]
              ]
              [. \node[l4,anchor=west,xshift=-9cm] {Tasks for V-L Generation};
                   [. \node[ppl,anchor=west,xshift=-10cm] {Seq2seq CMLM};
                   ]
                   [. \node[ppl,anchor=west,xshift=-10cm] {Decoupled-decoder-based Generation};
                   ]
                ]
              [. \node[l3,anchor=west,xshift=-9cm] {Downstream-driven Tasks};
                [. \node[ppl,anchor=west,xshift=-10cm] {Downstream Tasks for Pre-training};
                  ]
                  [. \node[ppl,anchor=west,xshift=-10cm] {Downstream-oriented Designed Tasks};
                  ]
              ]
            ]
        ]
        [. \node [l1,anchor=west,xshift=-6cm] {Downstream Evaluation};
            [. \node[ppl,anchor=west,xshift=-7cm] {V-L Understanding Tasks}; 
              [. \node[l4,anchor=west,xshift=-7cm] {Visual Question Answering (VQA)};
              ]
              [. \node[l4,anchor=west,xshift=-7cm] {Cross Modal Retrieval (CMR)};
              ]
              [. \node[l4,anchor=west,xshift=-7cm] {Natural Language for Visual Reasoning (NLVR)};
              ]
              [. \node[l4,anchor=west,xshift=-7cm] {Visual Entailment (VE)};
              ]
              [. \node[l4,anchor=west,xshift=-7cm] {Visual Commonsense Reasoning (VCR)};
              ]
              [. \node[l4,anchor=west,xshift=-7cm] {Referring Expression Comprehension (REC)};
              ]
              [. \node[l4,anchor=west,xshift=-7cm] {Visual Relationship Detection (VRD)};
              ]
              [. \node[l4,anchor=west,xshift=-7cm] {Visual Dialogue (VD)};
              ]
              [. \node[l4,anchor=west,xshift=-7cm] {Visual Linguistic Navigation (VLN))};
              ]
            ]
            [. \node[ppl,anchor=west,xshift=-7cm] {V-L Generation Tasks}; 
              [. \node[l3,anchor=west,xshift=-7cm] {Image Captioning (IC)};
              ]
              [. \node[l3,anchor=west,xshift=-7cm] {Novel Object Captioning (Nocaps)};
              ]
              [. \node[l3,anchor=west,xshift=-7cm] {Text-Caption (TextCaps)};
              ]
              [. \node[l3,anchor=west,xshift=-7cm] {Text Visual Question Answering (TextVQA)};
              ]
              [. \node[l3,anchor=west,xshift=-7cm] {Multimodal Machine Translation (MMT)};
              ]
            ]
            [. \node[ppl,anchor=west,xshift=-7cm] {Single-Modal Tasks};
              [. \node[l3,anchor=west,xshift=-7cm] {Image Classification};
              ]
              [. \node[l3,anchor=west,xshift=-7cm] {GLUE Benchmark Tasks};
              ]
            ]
        ]
    ]
\end{tikzpicture}
